Settle: Learning When to Stop Reasoning

Reasoning models often continue generating after their answers have settled. Settle learns when to stop from answer stability in completed traces. It trains the existing end-of-reasoning token while keeping other predictions close to the base model, and requires only ordinary decoding at inference. On MATH-500 with Qwen3-4B, Settle reduces token count by 40% with a 0.5-percentage-point decrease in accuracy. It gains 6.16 percentage points over supervised fine-tuning on the same traces shortened at their first stable answer, at nearly identical token counts. Its stopping score predicts whether a correct answer will remain correct. Settle extends the accuracy-token-count Pareto frontier of the evaluated stopping methods.

==> tables/agreement-sft.tex <==
% Validated selected full-response SFT cohorts.
SFT: stability-truncated, epoch 1 & 80.30 & 80.44 & 2,250\\
SFT: stability-truncated, epoch 2 & 87.45 & 87.53 & 2,345\\
\midrule
Settle, $w=0.10$ & 94.38 & 94.73 & 2,904\\
Settle, $w=0.25$ & 93.61 & 93.71 & 2,355\\


==> tables/anchor-main.tex <==
% Complete three-seed cohorts; ordinary-generation token counts.
Stability-truncated SFT & $\beta=0$ & $87.45\pm 2.56$ & $2,345\pm 75$\\
Stability-truncated SFT & $\beta=0.2$ & $88.25\pm 2.48$ & $2,564\pm 92$\\
Stability-truncated SFT & $\beta=1.0$ & $90.50\pm 1.94$ & $3,130\pm 122$\\
Stability-truncated SFT & $\beta=5.0$ & $92.96\pm 0.50$ & $3,884\pm 121$\\
\midrule
Settle, $w=0.25$ & $\lambda=0$ & $0.03\pm 0.06$ & $6,289\pm 6,642$\\
Settle, $w=0.25$ & $\lambda=0.2$ & $93.61\pm 0.24$ & $2,355\pm 62$\\


==> tables/baseline-development.tex <==
% Generated from validated raw outputs; do not edit numbers by hand.
Base (repeat evaluation) & 77.95 & 86.11 & 10,130\\
LSTM controller, $\tau=0.5$ & 30.38 & 30.38 & 2,169\\
LSTM controller, $\tau=0.9$ & 52.08 & 52.08 & 3,703\\
LSTM controller, $\tau=0.95$ & 56.60 & 56.60 & 4,190\\
LSTM controller, $\tau=0.99$ & 64.24 & 64.41 & 5,510\\
LSTM controller, $\tau=0.995$ & 68.06 & 68.23 & 6,095\\
LSTM controller, $\tau=0.999$ & 71.70 & 73.61 & 7,603\\
LSTM controller, $\tau=0.9995$ & 73.44 & 76.39 & 8,152\\
LSTM controller, $\tau=0.9999$ & 76.39 & 82.12 & 9,322\\
SFT: stability-truncated, $10^{-4}$, epoch 1 & 26.22 & 26.56 & 1,752\\
SFT: stability-truncated, $10^{-4}$, epoch 2 & 66.32 & 68.06 & 5,694\\
SFT: stability-truncated, $10^{-4}$, epoch 3 & 66.15 & 67.53 & 5,229\\
SFT: stability-truncated, $3\!\times\!10^{-4}$, epoch 1 & 47.92 & 48.44 & 3,337\\
SFT: stability-truncated, $3\!\times\!10^{-4}$, epoch 2 & 72.92 & 74.13 & 5,580\\
SFT: stability-truncated, $3\!\times\!10^{-4}$, epoch 3 & 71.53 & 72.92 & 5,183\\
Think Token Adjustment, $\alpha=0.2$ & 77.95 & 86.11 & 10,136\\
Think Token Adjustment, $\alpha=0.4$ & 78.12 & 86.11 & 10,133\\
Think Token Adjustment, $\alpha=0.6$ & 80.56 & 86.28 & 10,127\\
Think Token Adjustment, $\alpha=0.6$ (answer format) & 78.30 & 83.68 & 9,100\\
Think Token Adjustment, $\alpha=0.8$ & 78.65 & 86.46 & 10,108\\
Think Token Adjustment, $\alpha=1$ & 79.86 & 87.85 & 10,103\\


==> tables/baselines-main.tex <==
% Mean and sample SD across the documented evaluation runs.
\multicolumn{4}{l}{\textit{(a) Training objectives and reference anchoring}}\\
\addlinespace[2pt]
Base \cite{yang_qwen3_2025} & $93.89\pm 0.52$ & $95.23\pm 0.23$ & $4,828\pm 28$\\
SFT: shortest correct \cite{munkhbat_self-training_2025} & $94.13\pm 0.33$ & $\mathbf{95.30}\pm 0.14$ & $4,493\pm 70$\\
\addlinespace[2pt]
SFT: stability-truncated & $87.45\pm 2.56$ & $87.53\pm 2.58$ & $\mathbf{2,345}\pm 75^{\dagger}$\\
SFT: stability-truncated, $\beta=0.2$ & $88.25\pm 2.48$ & $88.52\pm 2.49$ & $2,564\pm 92$\\
SFT: stability-truncated, $\beta=1.0$ & $90.50\pm 1.94$ & $90.96\pm 1.83$ & $3,130\pm 122$\\
SFT: stability-truncated, $\beta=5.0$ & $92.96\pm 0.50$ & $93.86\pm 0.63$ & $3,884\pm 121$\\
Settle, $w=0.25$, $\lambda=0$ & $0.03\pm 0.06$ & $1.59\pm 1.08$ & $6,289\pm 6,642$\\
Settle, $w=0.10$ & $\mathbf{94.38}\pm 0.43$ & $94.73\pm 0.26$ & $2,904\pm 87$\\
Settle, $w=0.25$ & $93.61\pm 0.24$ & $93.71\pm 0.24$ & $2,355\pm 62^{\dagger}$\\
\addlinespace[2pt]
\multicolumn{4}{l}{\scriptsize $\dagger$ Token counts differ by 0.4\%; Settle gains 6.16 accuracy points over stability-truncated SFT.}\\
\midrule
\multicolumn{4}{l}{\textit{(b) Alternative stopping policies}}\\
\addlinespace[2pt]
LSTM controller \cite{liu_answer_2025} & $90.53\pm 2.47$ & $91.23\pm 3.02$ & $4,038\pm 486$\\
Halt Vector \cite{jayabahu_halt_2026} & $93.84\pm 0.08$ & $94.61\pm 0.08$ & $4,165\pm 68$\\
Token adjustment \cite{liu_answer_2025} & $93.54\pm 0.18$ & $\mathbf{94.93}\pm 0.18$ & $4,872\pm 42$\\
\quad + answer formatting & $87.06\pm 1.64$ & $87.88\pm 1.88$ & $4,036\pm 132$\\
DEER, default \cite{yang_dynamic_2025} & $\mathbf{94.81}\pm 0.15$ & $94.81\pm 0.15$ & $3,653\pm 10$\\
DEER, 100 trials \cite{yang_dynamic_2025} & $\mathbf{94.81}\pm 0.08$ & $94.81\pm 0.08$ & $3,153\pm 35$\\
DEER, $\theta=0.5$, $\rho=0.5$ \cite{yang_dynamic_2025} & $93.96\pm 0.12$ & $94.01\pm 0.08$ & $2,795\pm 29$\\
DEER, $\theta=0.95$, $\rho=0.25$ \cite{yang_dynamic_2025} & $92.72\pm 0.17$ & $92.75\pm 0.21$ & $2,658\pm 15$\\
\addlinespace[2pt]
Settle, $w=0.10$ & $94.38\pm 0.43$ & $94.73\pm 0.26$ & $2,904\pm 87$\\
Settle, $w=0.25$ & $93.61\pm 0.24$ & $93.71\pm 0.24$ & $\mathbf{2,355}\pm 62$\\
\midrule
\multicolumn{4}{l}{\textit{(c) Additional base and controller settings}}\\
\addlinespace[2pt]
Base (repeat evaluation) & $\mathbf{93.44}\pm 0.29$ & $\mathbf{94.95}\pm 0.25$ & $4,877\pm 26$\\
LSTM controller, $\tau=0.95$ & $87.28\pm 2.48$ & $87.68\pm 2.83$ & $\mathbf{3,302}\pm 390$\\
LSTM controller, $\tau=0.995$ & $91.35\pm 2.05$ & $92.17\pm 2.62$ & $4,262\pm 437$\\
LSTM controller, $\tau=0.9999$ & $93.42\pm 0.31$ & $94.78\pm 0.45$ & $4,817\pm 76$\\


==> tables/budget-curve.tex <==
2,048 & 78.01 & 1,950 \\
3,072 & 83.84 & 2,624 \\
4,096 & 87.70 & 3,115 \\
6,144 & 91.62 & 3,781 \\
8,192 & 93.47 & 4,198 \\
16,384 & 95.73 & 4,869 \\


==> tables/calibration-math-amc.tex <==
Base & 93.32 / 94.93 & 4,904 & 87.81 / 92.81 & 7,507\\
Settle, $w=0.01$ & 93.22 / 94.83 & 4,789 & 90.62 / 94.06 & 7,392\\
Settle, $w=0.025^\dagger$ & 93.98 / 95.13 & 4,410 & 89.38 / 91.88 & 6,896\\
Settle, $w=0.05$ & 94.58 / 95.28 & 3,643 & 88.44 / 90.62 & 5,897\\
Settle, $w=0.10$ & 94.18 / 94.58 & 2,890 & 89.06 / 89.69 & 4,822\\


==> tables/census.tex <==
Q3-4B MATH-500 8k & 500 & 87.8 & 0.21 & 85.6 / 94.4 & 4,151 / 1,704 \\
Q3-4B MATH-500 8k repeat & 500 & 86.6 & 0.21 & 83.0 / 93.0 & 4,185 / 1,724 \\
Q3-8B MATH-500 8k & 500 & 85.4 & 0.19 & 82.0 / 93.2 & 4,396 / 1,776 \\
Nemotron MATH-500 8k & 500 & 83.6 & 0.32 & 90.0 / 93.0 & 2,937 / 1,535 \\
Q3-4B MATH-500 16k & 500 & 87.6 & 0.20 & 94.0 / 95.4 & 4,809 / 2,065 \\


==> tables/controls.tex <==
Reference, $w=0.10$ & 3 & 93.96 & 94.38 & 2,961 \\
Reference, $w=0.25$ & 3 & 93.56 & 93.69 & 2,408 \\
Agreement, $w=0.25$ & 3 & 93.61 & 93.71 & 2,356 \\
Base cut at 2,560 & 1 & 35.89 & 80.77 & 2,314 \\
Shuffled labels & 1 & 86.75 & 86.80 & 1,296 \\
Shortest-correct SFT & 3 & 94.13 & 95.30 & 4,493 \\


==> tables/deer-budget-comparisons.tex <==
% Settle w & Settle-minus-DEER natural pp [pointwise 95% CI] & forced pp [pointwise 95% CI] & ordinary token savings (%).
\multicolumn{4}{l}{\textit{DEER $\theta=0.50,\ \rho=0.5$}} \\
0.10 & $+0.42\,[-0.18,\,+1.07]$ & $+0.72\,[+0.08,\,+1.42]$ & $-3.88$ \\
0.25 & $-0.35\,[-1.07,\,+0.38]$ & $-0.30\,[-1.00,\,+0.42]$ & $+15.73$ \\
\multicolumn{4}{l}{\textit{DEER $\theta=0.95,\ \rho=0.25$}} \\
0.10 & $+1.66\,[+0.82,\,+2.56]$ & $+1.97\,[+1.09,\,+2.93]$ & $-9.26$ \\
0.25 & $+0.89\,[-0.03,\,+1.86]$ & $+0.95\,[+0.03,\,+1.94]$ & $+11.37$ \\


==> tables/deer-budget-development.tex <==
% theta & rho & development natural accuracy (%) & ordinary probe-inclusive Token count & selected ceiling(s).
0.50 & 0.5 & 78.99 & 6,485 & $w=0.10$ \\
0.50 & 0.25 & 70.66 & 5,187 & --- \\
0.50 & 0.125 & 63.02 & 4,194 & --- \\
0.95 & 0.5 & 84.03 & 6,698 & --- \\
0.95 & 0.25 & 73.09 & 5,453 & $w=0.25$ \\
0.95 & 0.125 & 62.33 & 4,283 & --- \\


==> tables/deer.tex <==
% Archived single-run DEER sweep; explicit policy parameters.
0.95 & 10 & 0.80 & 94.83 & 3,688 & 118\\
0.90 & 10 & 0.80 & 94.78 & 3,530 & 115\\
0.85 & 10 & 0.80 & 94.83 & 3,561 & 115\\
0.80 & 10 & 0.80 & 94.88 & 3,475 & 115\\
0.70 & 10 & 0.80 & 94.63 & 3,480 & 114\\
0.50 & 10 & 0.80 & 94.93 & 3,470 & 114\\
0.95 & 100 & 0.80 & 94.78 & 3,157 & 229\\
0.95 & 10 & 0.50 & 94.73 & 3,294 & 118\\
0.50 & 10 & 0.50 & 94.33 & 3,152 & 114\\
0.50 & 100 & 0.50 & 94.33 & 2,784 & 199\\


==> tables/first-stable.tex <==
8,192 & First positive only & 92.77 & 3,257 \\
8,192 & All positive boundaries & 92.27 & 1,932 \\
16,384 & First positive only & 93.93 & 3,661 \\
16,384 & All positive boundaries & 93.37 & 2,063 \\


==> tables/lambda-perseed.tex <==
0.05 & 0 & 42 & 92.87 & 92.87 & 2,040.1\\
0.05 & 1 & 43 & 93.17 & 93.22 & 2,048.3\\
0.05 & 2 & 44 & 93.07 & 93.12 & 2,082.6\\
0.10 & 0 & 42 & 93.12 & 93.12 & 2,135.9\\
0.10 & 1 & 43 & 92.72 & 92.77 & 2,177.0\\
0.10 & 2 & 44 & 93.12 & 93.12 & 2,188.3\\
0.20 & 0 & 42 & 93.52 & 93.57 & 2,289.9\\
0.20 & 1 & 43 & 93.17 & 93.37 & 2,378.4\\
0.20 & 2 & 44 & 92.87 & 92.97 & 2,345.1\\
0.40 & 0 & 42 & 94.53 & 94.63 & 2,702.6\\
0.40 & 1 & 43 & 93.78 & 94.18 & 2,764.3\\
0.40 & 2 & 44 & 93.62 & 93.62 & 2,618.3\\


==> tables/lambda-sensitivity.tex <==
0.05 & 93.04 $\pm$ 0.15 & 93.07 $\pm$ 0.18 & 2,057 $\pm$ 23\\
0.10 & 92.99 $\pm$ 0.23 & 93.01 $\pm$ 0.20 & 2,167 $\pm$ 28\\
0.20 & 93.19 $\pm$ 0.33 & 93.31 $\pm$ 0.31 & 2,338 $\pm$ 45\\
0.40 & 93.98 $\pm$ 0.48 & 94.14 $\pm$ 0.50 & 2,695 $\pm$ 73\\


==> tables/latency.tex <==
Base & 1 & 1999.7 & 13.25 & 92 & 4,426 \\
Base & 32 & 323.7 & -- & 94 & 4,214 \\
Base & 100 & 160.5 & -- & 94 & 4,365 \\
Settle & 1 & 1165.2 & 7.66 & 91 & 2,602 \\
Settle & 32 & 301.9 & -- & 94 & 2,621 \\
Settle & 100 & 120.0 & -- & 90 & 2,670 \\
DEER & 1 & 1340.7 & $\approx 7.0$ & 95 & 2,884 \\
DEER & 32 & 520.7 & -- & 95 & 3,142 \\
DEER & 100 & 223.3 & -- & -- & 2,837 \\


==> tables/main.tex <==
Qwen3-4B & 8k & 92.92 & 92.79 & -0.13 [-0.95, +0.69] & 4,172 / 2,650 & 36.5 \\
Qwen3-4B & 16k & 95.23 & 94.73 & -0.50 [-1.27, +0.27] & 4,829 / 2,904 & 39.9 \\
Qwen3-8B & 16k & 95.67 & 95.45 & -0.22 [-0.94, +0.50] & 5,112 / 3,135 & 38.7 \\


==> tables/math-sample.tex <==
8k & 95.45 & 95.87 & +0.42 [-0.68, +1.55] & 3,493 / 2,045 & 41.5 \\
16k & 96.33 & 96.52 & +0.18 [-0.83, +1.22] & 3,803 / 2,179 & 42.7 \\


==> tables/models.tex <==
Qwen3-4B & MATH & 93.89 / 94.38 & 95.23 / 94.73 & -0.50 [-1.27, +0.27] & 39.9 \\
Qwen3-8B & MATH & 93.71 / 94.66 & 95.67 / 95.45 & -0.22 [-0.94, +0.50] & 38.7 \\
Nemotron-Nano-8B & MATH & 94.61 / 92.99 & 94.81 / 93.06 & -1.76 [-2.51, -1.04] & 33.3 \\
R1-Distill-Qwen-7B & MATH & 92.82 / 91.03 & 93.56 / 91.62 & -1.94 [-2.68, -1.22] & 31.6 \\


==> tables/native-current-correct.tex <==
Elapsed tokens & 0.552 [0.479, 0.630] & $0.500^{\dagger}$\\
Time-only spline & 0.551 [0.477, 0.630] & $0.500^{\dagger}$\\
Settle, $w=0.10$ & 0.702 [0.645, 0.760] & 0.695 [0.624, 0.764]\\
Settle, $w=0.25$ & 0.715 [0.659, 0.771] & 0.706 [0.635, 0.774]\\


==> tables/native-position-main.tex <==
Base native score & 0.532 [0.508, 0.556] & 0.507 [0.484, 0.530] & 0.495 [0.445, 0.547] \\
Elapsed tokens & 0.618 [0.583, 0.655] & $0.500^{\dagger}$ & $0.500^{\dagger}$\\
Time-only spline & 0.618 [0.583, 0.654] & $0.500^{\dagger}$ & $0.500^{\dagger}$\\
Settle, $w=0.10$ & 0.831 [0.811, 0.851] & 0.807 [0.782, 0.831] & 0.695 [0.624, 0.764]\\
Settle, $w=0.25$ & 0.838 [0.819, 0.857] & 0.818 [0.793, 0.842] & 0.706 [0.635, 0.774]\\


==> tables/native-position-strata.tex <==
$[0,1024)$ & 6,798 & 0.680 [0.657, 0.703] & 0.842 [0.821, 0.863] & 0.853 [0.831, 0.873]\\
$[1024,2048)$ & 4,667 & 0.534 [0.508, 0.560] & 0.824 [0.787, 0.858] & 0.832 [0.795, 0.867]\\
$[2048,4096)$ & 3,678 & 0.452 [0.421, 0.483] & 0.766 [0.719, 0.814] & 0.771 [0.723, 0.820]\\
$[4096,8192)$ & 2,014 & 0.489 [0.442, 0.537] & 0.743 [0.687, 0.798] & 0.755 [0.700, 0.809]\\
$[8192,16384)$ & 742 & 0.500 [0.500, 0.500] & 0.681 [0.572, 0.782] & 0.682 [0.575, 0.782]\\


==> tables/native-time-matched.tex <==
64 tokens & 17,843 & 1,024,057 & 0.506 [0.497, 0.516] & 0.805 [0.781, 0.826] & 0.816 [0.793, 0.838]\\
128 tokens & 17,886 & 2,048,420 & 0.514 [0.504, 0.524] & 0.805 [0.782, 0.827] & 0.817 [0.793, 0.838]\\
256 tokens & 17,899 & 4,100,706 & 0.522 [0.512, 0.532] & 0.806 [0.783, 0.827] & 0.817 [0.794, 0.839]\\
Exact token count & 12,106 & 16,267 & 0.500 [0.500, 0.500] & 0.807 [0.782, 0.831] & 0.818 [0.793, 0.842]\\


==> tables/self-closure.tex <==
8,192 & 0 & 86.45 & 1,767 \\
8,192 & 1 & 86.60 & 1,684 \\
16,384 & 0 & 88.15 & 1,923 \\


==> tables/settle-sft-comparisons.tex <==
% SFT beta & Settle-minus-SFT natural accuracy pp [95% CI] & forced accuracy pp [95% CI] & ordinary token savings (%).
\multicolumn{4}{l}{\textit{Settle $w=0.10$}} \\
0 & $+6.93\,[+5.52,\,+8.43]$ & $+7.20\,[+5.79,\,+8.68]$ & $-23.81$ \\
0.2 & $+6.12\,[+4.77,\,+7.56]$ & $+6.21\,[+4.84,\,+7.65]$ & $-13.26$ \\
1.0 & $+3.88\,[+2.71,\,+5.10]$ & $+3.77\,[+2.58,\,+5.00]$ & $+7.22$ \\
5.0 & $+1.42\,[+0.42,\,+2.49]$ & $+0.87\,[-0.13,\,+1.92]$ & $+25.25$ \\
\multicolumn{4}{l}{\textit{Settle $w=0.25$}} \\
0 & $+6.16\,[+4.70,\,+7.68]$ & $+6.17\,[+4.70,\,+7.70]$ & $-0.43$ \\
0.2 & $+5.35\,[+3.93,\,+6.81]$ & $+5.19\,[+3.78,\,+6.64]$ & $+8.12$ \\
1.0 & $+3.11\,[+1.81,\,+4.42]$ & $+2.74\,[+1.44,\,+4.05]$ & $+24.74$ \\
5.0 & $+0.65\,[-0.54,\,+1.84]$ & $-0.15\,[-1.32,\,+1.00]$ & $+39.36$ \\


==> tables/stop-readouts.tex <==
Native closing-token probability & 0.532 & 0.846 \\
Linear probe: final hidden state & 0.803 & 0.854 \\
Linear probe: middle hidden state & 0.831 & 0.833 \\


==> tables/suite.tex <==
GSM8K & 1319 & 1 & 95.1 / 94.5 & -0.7 & 2,053 / 1,167 & 43.2 \\
AMC23 & 40 & 8 & 93.4 / 90.8 & -2.6 & 7,617 / 4,903 & 35.6 \\
Minerva & 272 & 1 & 48.2 / 44.5 & -3.7 & 6,536 / 3,327 & 49.1 \\
OlympiadBench & 674 & 1 & 66.6 / 70.4 & +3.8 & 9,024 / 5,750 & 36.3 \\
GPQA-Diamond & 198 & 1 & 55.6 / 55.9 & +0.3 & 8,565 / 7,433 & 13.2 \\


==> tables/training-grid.tex <==
\multicolumn{5}{l}{\emph{MATH-500}}\\
Original & Agreement & $94.21\pm 0.15$ & $94.66\pm 0.14$ & $2{,}943\pm 49$\\
Original & Reference & $94.31\pm 0.28$ & $94.85\pm 0.16$ & $2{,}961\pm 109$\\
Broader & Agreement & $94.01\pm 0.21$ & $94.38\pm 0.17$ & $3{,}073\pm 73$\\
Broader & Reference & $94.08\pm 0.46$ & $94.98\pm 0.39$ & $3{,}169\pm 164$\\

